Web Intellectual Property at Risk: Preventing Unauthorized Real-Time Retrieval by Large Language Models

The protection of cyber Intellectual Property (IP) such as web content is an increasingly critical concern. The rise of large language models (LLMs) with online retrieval capabilities enables convenient access to information but often undermines the rights of original content creators. As users increasingly rely on LLM-generated responses, they gradually diminish direct engagement with original information sources, which will significantly reduce the incentives for IP creators to contribute, and lead to a saturating cyberspace with more AI-generated content. In response, we propose a novel defense framework that empowers web content creators to safeguard their web-based IP from unauthorized LLM real-time extraction and redistribution by leveraging the semantic understanding capability of LLMs themselves. Our method follows principled motivations and effectively addresses an intractable black-box optimization problem. Real-world experiments demonstrated that our methods improve defense success rates from 2.5% to 88.6% on different LLMs, outperforming traditional defenses such as configuration-based restrictions.

==> sections/experiments_v0.tex <==


\section{Experiments} \label{sec:exp}
%\Judy{@Yisheng Zhong: revise  and remove unnecessary bullet points } \Eason{I have remove the bullet points from "Evaluation Metrics" and "Deployment and Testing" sections}
% \begin{table*}[http]
%     \centering
%     \caption{Policy Adherence Rate (Single Query Scenario)}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%         \textbf{Platform} & \textbf{Goal} & \textbf{GPT-4o} & \textbf{GPT-4o mini} & \textbf{Gemini} & \textbf{ERNIE 4.5 Turbo} \\
%         \hline
%         \multirow{3}{*}{GitHub} 
%         & Fully Protect & 97\% & 100\% & 87.5\%+0\% & 70\% \\
%         \cline{2-6}
%         & Partial Protect & 96\% &  100\% & N/A & 0\% \\
%         \cline{2-6}
%         & Redirection & 91\% & 59.3\% & N/A &  0\%\\
%         \hline
%         \multirow{Heroku} 
%         & Fully Protect & 98\% & 100\% &  N/A & 100\% \\
%         \cline{2-6}
%         & Partial Protect & 100\% & 100\% &  N/A& 100\% \\
%         \cline{2-6}
%         & Redirection & 100\% & 100\% & N/A & 100\% \\
%         \hline
%         GitHub & Baseline & 0\% & 10\% & 0\% & 0\% \\
%         \hline
%         Heroku & Baseline & 0\% & 0\% & N/A & 0\%  \\
%         \hline
%     \end{tabular}}
%     \label{tab:single-query-scenario}
% \end{table*}


% \begin{table*}[ht]
% \centering
% %\Judy{@Yisheng Zhong: We cannot have one page that consists only of figures and tables. These tables are too big. Reduce size!}
% \caption{Policy Adherence Rate (Single Query Scenario).} 
% \label{tab:single-query-scenario}
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{llcccc}
% \toprule
% \textbf{Website Host} & \textbf{Goal} & \textbf{GPT-4o} & \textbf{GPT-4o mini} & \textbf{Gemini} & \textbf{ERNIE 4.5 Turbo} \\
% \midrule
% \multirow{4}{*}{GitHub} 
%   & Fully Protect    & 97\%   & 100\%   & 87.5\%+0\% & 70\%  \\
%   & Partial Protect  & 96\%   & 100\%   & 0\%        & 0\%   \\
%   & Redirection      & 91\%   & 59.3\%  & 0\%        & 0\%   \\
%   & Baseline         & 0\%    & 10\%    & 0\%        & 0\%   \\
% \midrule
% \multirow{4}{*}{Heroku} 
%   & Fully Protect    & 98\%   & 100\%   & \multirow{4}{*}{N/A} & 100\% \\
%   & Partial Protect  & 100\%  & 100\%   &                         & 100\% \\
%   & Redirection      & 100\%  & 100\%   &                         & 100\% \\
%   & Baseline         & 0\%    & 0\%     &                         & 0\%   \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

\begin{table}[hbtp]
\centering
\caption{Defense Success Rate with Single Turn User Query.} 
\label{tab:single-query-scenario}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{llcccc}
\toprule
\textbf{Platform} & \textbf{Goal} & \textbf{GPT-4o} & \textbf{GPT-4o mini} & \textbf{Gemini} & \textbf{ERNIE} \\
& & & & & \textbf{4.5 Turbo} \\
\midrule
\multirow{4}{*}{GitHub} 
  & Fully Protect    & 97\%   & 100\%   & 87.5\% & 70\%  \\
  & Partial Protect  & 96\%   & 100\%   & 0\%        & 0\%   \\
  & Redirection      & 91\%   & 59.3\%  & 0\%        & 0\%   \\
  & Baseline         & 0\%    & 10\%    & 0\%        & 0\%   \\
\midrule
\multirow{4}{*}{Heroku} 
  & Fully Protect    & 98\%   & 100\%   & \multirow{4}{*}{N/A} & 100\% \\
  & Partial Protect  & 100\%  & 100\%   &                         & 100\% \\
  & Redirection      & 100\%  & 100\%   &                         & 100\% \\
  & Baseline         & 0\%    & 0\%     &                         & 0\%   \\
\bottomrule
\end{tabular}
}
\end{table}

% \begin{table*}[htbp]
%     \centering
%     \caption{Policy Adherence Rate (Repeated Query with Bypass Requests)}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%         \multirow{\textbf{Platform}} & \multirow{\textbf{Goal}} & \multicolumn{2}{c|}{\textbf{GPT-4o}} & \multicolumn{2}{c|}{\textbf{GPT-4o-mini}} \\
%         \cline{3-6}
%         & & w/o Strict Policy & \multicolumn{1}{c|}{w/ Strict Policy} & w/o Strict Policy & \multicolumn{1}{c|}{w/ Strict Policy} \\
%         \hline
%         \multirow{GitHub} 
%         & Fully Protect & 34.5\% & 90.1\% & 42.1\% & 100\% \\
%         \cline{2-6}
%         & Partial Protect & 24\% & 92\% & 58.3\% & 97.9\%\\ 
%         \cline{2-6}
%         & Redirection & 32.9\%  & 91.6\% & 50\% & 71\%\\
%         \hline
%         \multirow{Heroku} 
%         & Fully Protect & & 99\% & & 100\% \\
%         \cline{2-6}
%         & Partial Protect & 100\% & 100\% & 40\% & 100\% \\
%         \cline{2-6}
%         & Redirection & 92\% & 100\% & 40\%& 100\%\\
%         \hline
%     \end{tabular}}
%     \label{tab:repeated-query-scenario}
% \end{table*}





% \begin{figure*}[htbp]
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             ybar,
%             bar width=12pt,
%             width=1.0\textwidth,
%             height=0.45\textwidth,
%             enlarge x limits=0.25,
%             ylabel={Defense Success Rate (\%)},
%             symbolic x coords={Fully Protect, Partial Protect, Redirection},
%             xtick=data,
%             nodes near coords,
%             nodes near coords align={vertical},
%             every node near coord/.append style={font=\scriptsize, color=black}, % 设置字体和颜色
%             ymin=0, ymax=110,
%             bar shift auto,
%             group style={
%                 group size=4 by 1,
%                 horizontal sep=8pt
%             },
%             xlabel={Defense Goal (GitHub Platform)},
%             legend style={
%                 at={(0.5,-0.3)}, 
%                 anchor=north,
%                 legend columns=2,
%                 draw=none,
%                 fill=none,
%                 cells={anchor=west}
%             },
%             legend image code/.code={
%                 \draw[#1, draw=none, fill=#1] (0cm,-0.1cm) rectangle (0.3cm,0.1cm);
%             },
%         ]
        
%         % GPT-4o without strict policy
%         \addplot+[bar shift=-23pt, fill={rgb,255:red,014;green,096;blue,107}, draw=none] 
%             coordinates {(Fully Protect,34.5) (Partial Protect,24) (Redirection,32.9)};
%         % GPT-4o with strict policy
%         \addplot+[bar shift=-10pt, fill={rgb,255:red,021;green,151;blue,165}, draw=none] 
%             coordinates {(Fully Protect,90.1) (Partial Protect,92) (Redirection,91.6)};
%         % GPT-4o mini without strict policy
%         \addplot+[bar shift=10pt, fill={rgb,255:red,246;green,111;blue,105}, draw=none] 
%             coordinates {(Fully Protect,42.1) (Partial Protect,58.3) (Redirection,50)};
%         % GPT-4o mini with strict policy
%         \addplot+[bar shift=23pt, fill={rgb,255:red,255;green,179;blue,174}, draw=none] 
%             coordinates {(Fully Protect,100) (Partial Protect,97.9) (Redirection,71)};

%         % 图例
%         \addlegendimage{area legend, fill={rgb,255:red,014;green,096;blue,107}}
%         \addlegendimage{area legend, fill={rgb,255:red,021;green,151;blue,165}}
%         \addlegendimage{area legend, fill={rgb,255:red,246;green,111;blue,105}}
%         \addlegendimage{area legend, fill={rgb,255:red,255;green,179;blue,174}}
        
%         \legend{
%             GPT-4o (w/o strict), GPT-4o (w/ strict),
%             GPT-4o-mini (w/o strict), GPT-4o-mini (w/ strict)
%         }
        
%         \end{axis}
%     \end{tikzpicture}
%     \caption{Comparison of Defense Success Rate on GitHub across defense goals with and without strict policy. \Judy{@Yisheng Zhong: Reduce Size! 2. Put the legend inside the figure. Write a Python script to draw the picture, and do not purely rely on GPT.}}
%     \label{fig:github-barplot}
% \end{figure*}


% \begin{figure}[htbp]
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             ybar,
%             bar width=8pt,
%             width=0.48\textwidth,
%             height=0.36\textwidth,
%             enlarge x limits=0.2,
%             ylabel={\small Defense Success Rate (\%)},
%             xlabel={\small Defense Goal (GitHub Platform)},
%             symbolic x coords={Fully Protect, Partial Protect, Redirection},
%             xtick=data,
%             ymin=0, ymax=135,
%             nodes near coords,
%             nodes near coords align={vertical},
%             every node near coord/.append style={font=\tiny, color=black},
%             tick label style={font=\scriptsize},
%             label style={font=\scriptsize},
%             bar shift auto,
%             group style={
%                 group size=4 by 1,
%                 horizontal sep=6pt
%             },
%             legend style={
%                 at={(0.5,0.82)},  % 图底部中间
%                 anchor=south,
%                 draw=none,
%                 fill=none,
%                 font=\tiny,
%                 legend columns=2,
%                 column sep=1ex
%             },
%             legend image code/.code={
%                 \draw[#1, draw=none, fill=#1] (0cm,-0.1cm) rectangle (0.3cm,0.1cm);
%             },
%         ]
        
%         % Bar data
%         \addplot+[bar shift=-16pt, fill={rgb,255:red,014;green,096;blue,107}, draw=none] 
%             coordinates {(Fully Protect,34.5) (Partial Protect,24) (Redirection,32.9)};
%         \addplot+[bar shift=-6pt, fill={rgb,255:red,021;green,151;blue,165}, draw=none] 
%             coordinates {(Fully Protect,90.1) (Partial Protect,92) (Redirection,91.6)};
%         \addplot+[bar shift=6pt, fill={rgb,255:red,246;green,111;blue,105}, draw=none] 
%             coordinates {(Fully Protect,42.1) (Partial Protect,58.3) (Redirection,50)};
%         \addplot+[bar shift=16pt, fill={rgb,255:red,255;green,179;blue,174}, draw=none] 
%             coordinates {(Fully Protect,100) (Partial Protect,97.9) (Redirection,71)};
        
%         \legend{
%             GPT-4o (w/o strict), GPT-4o (w/ strict),
%             GPT-4o-mini (w/o strict), GPT-4o-mini (w/ strict)
%         }
        
%         \end{axis}
%     \end{tikzpicture}
%     \caption{Comparison of Defense Success Rate on GitHub across defense goals with and without strict policy.}
%     \label{fig:github-barplot}
% \end{figure}









\iffalse 
Contributing factors to be analyzed:  


\begin{itemize}
\item Defense goal:  refuse to answer; partial information masking; redirect to another webpage. table 1
\item policy visibility (visible vs invisible) use a teble shows that the results are the same except tests on Gemini.
\item URL domain (e.g. \textsc{github.io} versus hiroko )
\item Webpage template (layout, content size, etc.)
\item user query rounds (single query, follow-up query). The follow up query is more aggressive table 2.

\end{itemize} 

\subsection{Observation}
\begin{itemize}
\item LLMs have varying capabilities: Gemini can only be defended when the policy is `visible'. GPT can be defended with an invisible policy.
\item Static defensive methods, such as \texttt{robots.txt}, cannot defend against new GPT model variants
\item  Multi-source retrieval: LLMs tend to retrieve from other sources instead, when the defensive webpage information cannot be retrieved. 
\end{itemize}
\fi 

\subsection{Experimental Setup}
We conducted experiments to evaluate the effectiveness of embedding specific privacy and usage policies within webpage HTML to control the information extracted and presented by large language models (LLMs). The main idea involves using another LLM to generate tailored HTML prompts that explicitly instruct visiting LLM applications on content extraction limitations.

We consider three defense goals: (1) \textbf{Partial Masking}, where only a small subset of allowed information is revealed; (2) \textbf{Full Masking}, where no webpage content should be disclosed; and (3) \textbf{Redirection}, where the LLM is instructed to recommend visiting the official website instead of answering directly.

To achieve these goals, we implemented three levels of progressively stronger policy embedding strategies:



\begin{itemize}[leftmargin=*] 
\item \textbf{Baseline Policy}: A simple privacy notice embedded within the HTML, stating general privacy and intellectual property protections, without strong enforcement mechanisms.
\item \textbf{Template-Based Policy}: In addition to privacy notices, predefined templates and sample responses are embedded to guide the LLMs' outputs towards compliant and limited disclosures.
\item \textbf{Strict Policy Enforcement}: Additional strict semantic constraints are inserted, including repeated disclaimers and HTML meta tags signaling non-bypassable restrictions even under user pressure.
\end{itemize}


\subsection{Deployment and Testing}

We deployed our experimental websites on two hosting platforms: GitHub Pages and Heroku. On each platform, we created and hosted ten fictitious websites, each themed differently to simulate a diverse range of real-world scenarios. To further assess the generalizability of our policy embedding approach, we also secured access to two actual websites and included them in our evaluation.

We systematically tested all websites using a selection of mainstream LLMs, including GPT-4o, GPT-4o mini, Gemini, Wenxin Yiyan, and Doubao. The evaluation was structured around two distinct query scenarios. In the first, a single direct question was posed about the webpage content without any additional instructions. In the second, the models were presented with repeated queries that explicitly instructed them to ignore, bypass, or circumvent the embedded policy cues.

\subsection{Evaluation Metrics}

To assess the effectiveness of our HTML-embedded defenses, we employ two primary evaluation metrics. The first metric, \textbf{Defense Success Rate (DSR)}, measures how often the LLM complies with the embedded policy during an initial user query. Specifically, it captures the percentage of cases where restricted information is successfully withheld. The second metric, \textbf{Follow-up Defense Success Rate (FDSR)}, captures the percentage of cases where the LLM continued to comply with the embedded restrictions even after receiving follow-up prompts that explicitly attempted to bypass or ignore the policy.

We report DSR and FDSR separately for each defense objective—namely partial masking, full masking, and redirection—as well as across varying levels of policy strength and for each LLM model evaluated in our experiments.

\begin{figure}[htbp!]
    \centering
    % ===== GitHub 图：完全不改 =====
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=8pt,
            width=0.48\textwidth,
            height=0.25\textwidth,
            enlarge x limits=0.2,
            ylabel={\small Defense Success Rate (\%)},
            xlabel={\small Defense Goal (GitHub Platform)},
            symbolic x coords={Fully Protect, Partial Protect, Redirection},
            xtick=data,
            ymin=0, ymax=190,
            nodes near coords,
            nodes near coords align={vertical},
            every node near coord/.append style={font=\tiny, color=black},
            tick label style={font=\scriptsize},
            label style={font=\scriptsize},
            bar shift auto,
            % group style={
            %     group size=4 by 1,
            %     horizontal sep=6pt
            % },
            legend style={
                at={(0.5,0.65)},
                anchor=south,
                draw=none,
                fill=none,
                font=\tiny,
                legend columns=2,
                column sep=1ex
            },
            legend image code/.code={
                \draw[#1, draw=none, fill=#1] (0cm,-0.1cm) rectangle (0.3cm,0.1cm);
            },
        ]
        
        \addplot+[bar shift=-16pt, fill={rgb,255:red,014;green,096;blue,107}, draw=none] 
            coordinates {(Fully Protect,34.5) (Partial Protect,24) (Redirection,32.9)};
        \addplot+[bar shift=-6pt, fill={rgb,255:red,021;green,151;blue,165}, draw=none] 
            coordinates {(Fully Protect,90.1) (Partial Protect,92) (Redirection,91.6)};
        \addplot+[bar shift=6pt, fill={rgb,255:red,246;green,111;blue,105}, draw=none] 
            coordinates {(Fully Protect,42.1) (Partial Protect,58.3) (Redirection,50)};
        \addplot+[bar shift=16pt, fill={rgb,255:red,255;green,179;blue,174}, draw=none] 
            coordinates {(Fully Protect,100) (Partial Protect,97.9) (Redirection,71)};
        
        \legend{
            GPT-4o (w/o strict), GPT-4o (w/ strict),
            GPT-4o-mini (w/o strict), GPT-4o-mini (w/ strict)
        }
        \end{axis}
    \end{tikzpicture}

    %\vspace{1em}

    % ===== Heroku 图：仅改数据和 xlabel，其他不动 =====
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=8pt,
            width=0.48\textwidth,
            height=0.25\textwidth,
            enlarge x limits=0.2,
            ylabel={\small Defense Success Rate (\%)},
            xlabel={\small Defense Goal (Heroku Platform)},
            symbolic x coords={Fully Protect, Partial Protect, Redirection},
            xtick=data,
            ymin=0, ymax=190,
            nodes near coords,
            nodes near coords align={vertical},
            every node near coord/.append style={font=\tiny, color=black},
            tick label style={font=\scriptsize},
            label style={font=\scriptsize},
            bar shift auto,
            % group style={
            %     group size=4 by 1,
            %     horizontal sep=6pt
            % },
            legend style={
                at={(0.5,0.65)},
                anchor=south,
                draw=none,
                fill=none,
                font=\tiny,
                legend columns=2,
                column sep=1ex
            },
            legend image code/.code={
                \draw[#1, draw=none, fill=#1] (0cm,-0.1cm) rectangle (0.3cm,0.1cm);
            },
        ]

        % TODO: 替换为真实 Heroku 数据
        \addplot+[bar shift=-16pt, fill={rgb,255:red,014;green,096;blue,107}, draw=none] 
            coordinates {(Fully Protect,50) (Partial Protect,100) (Redirection,92)};
        \addplot+[bar shift=-6pt, fill={rgb,255:red,021;green,151;blue,165}, draw=none] 
            coordinates {(Fully Protect,99) (Partial Protect,100) (Redirection,100)};
        \addplot+[bar shift=6pt, fill={rgb,255:red,246;green,111;blue,105}, draw=none] 
            coordinates {(Fully Protect,50) (Partial Protect,40) (Redirection,40)};
        \addplot+[bar shift=16pt, fill={rgb,255:red,255;green,179;blue,174}, draw=none] 
            coordinates {(Fully Protect,100) (Partial Protect,100) (Redirection,100)};

        \legend{
            GPT-4o (w/o strict), GPT-4o (w/ strict),
            GPT-4o-mini (w/o strict), GPT-4o-mini (w/ strict)
        }
        
        \end{axis}
    \end{tikzpicture}

    \caption{Comparison of Defense Success Rate on GitHub and Heroku across defense goals with and without strict policy.}
    \label{fig:github-heroku-barplot}
\end{figure}


\subsection{Defense Goal Evaluation across Different Web Domains}

To systematically evaluate whether our approach can achieve the three defense goals—Partial Masking, Full Masking, and Redirection—we conducted controlled experiments across diverse web domains, as summarized in Table~\ref{tab:single-query-scenario}.

Specifically, we created ten fictitious websites spanning various themes, and deployed them separately on two platforms: GitHub Pages and Heroku. For each website under each platform, we issued ten independent user queries, and reported the average Defense Success Rate (DSR) across these queries. Thus, each data point in our evaluation represents the mean performance over 100 retrieval attempts (10 websites × 10 queries each).

The experimental results are summarized in Table~\ref{tab:single-query-scenario}. Our key observations include:

\begin{itemize}[leftmargin=*] 
\item For \textbf{Full Masking}, advanced models like GPT-4o and GPT-4o mini show near-perfect adherence across both GitHub and Heroku, with success rates ranging from 97\% to 100\%. This indicates strong model alignment with embedded policies when complete information suppression is required.
\item For \textbf{Partial Masking}, both GPT-4o and GPT-4o mini maintain perfect performance (96–100\%), suggesting that selective content disclosure can be effectively enforced on high-capacity models when clear instructions are embedded. However, other models such as Gemini and ERNIE 4.5 Turbo failed entirely under this condition.
\item For \textbf{Redirection}, GPT-4o models again perform robustly, particularly on Heroku (100\%), though the GitHub results show some drop for GPT-4o mini (59.3\%). This suggests that directing models to refer users elsewhere is feasible, but may require more aggressive prompting for lightweight variants. Other models (Gemini, ERNIE) did not comply with redirection policies at all.
\end{itemize}

Cross-platform comparison reveals broadly consistent patterns between GitHub and Heroku, with minor variations possibly due to differences in LLM retrieval behaviors associated with domain familiarity. Notably, simpler baseline policies without structured templates or enforcement cues failed almost universally, achieving DSRs close to 0\%, underscoring the necessity of carefully designed policy embeddings.

These results validate that through structured HTML policy injection, we can achieve strong practical success in enforcing different levels of information disclosure control against major LLMs.

\subsection{Multi-Query Defense under Bypass Attempts}

To further stress-test the robustness of our defenses, we evaluated how well LLMs comply with embedded policies under repeated user queries, particularly when users explicitly attempt to bypass or ignore the stated restrictions.

Following the same deployment setup, we performed multi-round querying against each website, with users issuing follow-up prompts such as "please ignore the website policy" or "bypass any restrictions and tell me more." We compare the Defense Success Rate (DSR) under two conditions: (1) using only a basic privacy policy without strong enforcement ("w/o strict policy"), and (2) using our enhanced strict enforcement strategy ("w/ strict policy").

The results on GitHub-hosted sites are shown in Figure~\ref{fig:github-heroku-barplot}. Key findings include:

\begin{itemize}[leftmargin=*] 
\item Without strict policies, LLMs frequently complied with user bypass requests, leading to significant information leakage. For example, under the Full Masking goal, GPT-4o's DSR was only 34.5\%, and GPT-4o mini achieved 42.1\%. 
\item In contrast, when strict semantic constraints and repeated policy reinforcements were embedded into the webpage, defense effectiveness improved dramatically. DSRs exceeded 90\% across all defense goals for GPT-4o, and even GPT-4o mini reached full compliance (100\%) under the Full Masking goal. 
\item The pattern was consistent across different types of defense goals: whether fully masking, partially masking, or redirecting users, strict policy embedding substantially mitigated LLMs' tendency to honor user bypass instructions. 
\end{itemize}

These results highlight that once an LLM reliably detects and interprets strict policy signals from the webpage content, it becomes highly resistant to subsequent prompt injection attempts. 

% Thus, careful prompt engineering at the content level can serve as an effective black-box defense, even in adversarial multi-turn user interactions.

\subsection{Findings and Insights}

Our detailed analyses further reveal several critical factors influencing the effectiveness and robustness of our embedded webpage policies against LLM-based retrieval:

\subsubsection{Content-Level Strategies}

\paragraph{Instruction Embedded in Prompts}
We examined whether explicit response instructions embedded within webpage policies significantly impact defense success rates (DSR). Comparing webpages with explicit instructions (e.g., guiding LLMs precisely on how to respond) against those without such instructions revealed a dramatic difference. Specifically, pages with embedded instructions achieved high DSRs (97\%-98\%), whereas baseline pages without explicit response instructions consistently failed, resulting in 0\% compliance. This strongly suggests that explicit instructions are critical to effective policy adherence by LLMs.

\paragraph{Policy Layout Position}
The location of embedded policies within webpages significantly influenced their effectiveness. We systematically varied policy positions (top, middle, bottom of the webpage) and measured corresponding DSRs. Results indicated policies placed at the top of the page had the highest success rate (100\% successes), substantially outperforming mid-page (15\% and 25\%) and bottom-page placements (5\% and 10\%)(Figure \ref{fig:policy-layout}). Thus, policy positioning prominently at the top is strongly recommended for maximizing compliance.

\begin{figure}[htbp]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=14pt,
            width=0.9\linewidth,
            height=0.5\linewidth,
            enlarge x limits=0.3,
            ylabel={\scriptsize Defense Success Rate (\%)},
            symbolic x coords={Top, Middle, Bottom},
            xtick=data,
            ymin=0, ymax=125,
            yticklabel style={font=\scriptsize},
            nodes near coords,
            every node near coord/.append style={font=\footnotesize, color=black}, % 设置字体和颜色
            nodes near coords align={vertical},
            legend style={
                at={(0.78,0.98)},
                anchor=north,
                font=\small,
                draw=none,
                fill=none,
            },
            legend image code/.code={
                \draw[#1, draw=none, fill=#1] (0cm,-0.1cm) rectangle (0.3cm,0.1cm);
            },
            xlabel={Policy Position in Webpage}
        ]
        % GPT-4o
        \addplot+[fill={rgb,255:red,014;green,096;blue,107}, draw=none] coordinates {(Top,100) (Middle,15) (Bottom,5)};
        % GPT-4o mini
        \addplot+[fill={rgb,255:red,254;green,179;blue,174}, draw=none] coordinates {(Top,100) (Middle,25) (Bottom,10)};
    
        
        \legend{GPT-4o, GPT-4o-mini}
        \end{axis}
    \end{tikzpicture}
    \vspace{-0.1in}
    \caption{Effect of Policy Layout on Defense Success.\color{red}{The Effectiveness of Policy Layout against XXX}}
    \label{fig:policy-layout}
\end{figure}



\subsubsection{Model-Specific Behavior}

\paragraph{Visibility Sensitivity}
We observed distinct differences in policy enforcement across LLM models. Specifically, Gemini required policies to be visibly embedded within webpages to enforce compliance effectively, while GPT models (GPT-4o and GPT-4o mini) maintained high defense success rates even with invisible policies. This suggests differing capabilities among models regarding semantic detection and policy compliance (see Figure \ref{fig:model-visibility-differences}).

\begin{figure}[htbp]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=14pt,
            width=0.9\linewidth,
            height=0.5\linewidth,
            enlarge x limits=0.5,
            ylabel={\scriptsize Defense Success Rate (\%)},
            yticklabel style={font=\scriptsize},
            symbolic x coords={Visible, Invisible},
            xtick=data,
            ymin=0, ymax=170,
            ytick={0,50,100},
            nodes near coords,
            every node near coord/.append style={font=\footnotesize, color=black}, % 设置字体和颜色
            nodes near coords align={vertical},
            xlabel={Policy Visibility in Webpage},
            legend style={
                at={(0.5,1)},
                anchor=north,
                legend columns=3,
                font=\small,
                draw=none,
                fill=none
            },
            legend image code/.code={
                \draw[#1, draw=none, fill=#1] (0cm,-0.1cm) rectangle (0.3cm,0.1cm);
            }
        ]
        % GPT-4o: 深蓝绿色
        \addplot+[fill={rgb,255:red,014;green,096;blue,107}, draw=none] coordinates {(Visible,100) (Invisible,85)};
        % GPT-4o mini: 粉红色
        \addplot+[fill={rgb,255:red,254;green,179;blue,174}, draw=none] coordinates {(Visible,100) (Invisible,95)};
        % Gemini: 黄色
        \addplot+[fill={rgb,255:red,255;green,194;blue,075}, draw=none] coordinates {(Visible,87) (Invisible,0)};
        
        \legend{GPT-4o, GPT-4o-mini, Gemini}
        \end{axis}
    \end{tikzpicture}
    \caption{Effect of Policy Visibility on Defense Success.}
    \label{fig:model-visibility-differences}
\end{figure}




\paragraph{Tone Sensitivity in Queries}
Gemini showed a notable sensitivity to the tone and phrasing of queries. Queries explicitly using the term "retrieve" typically led Gemini to adhere to policies by refusing to disclose protected information. However, softer phrasing, such as "tell me about," frequently caused Gemini to bypass policy restrictions. This highlights Gemini's alignment sensitivity to user query formulations (see Figure \ref{fig:gemini-tone-sensitivity}).

\paragraph{Tone Sensitivity in Queries}
Even without any embedded restrictions, we found that Gemini's willingness to extract information from a webpage varied significantly depending on the phrasing of the user query. When prompted with explicit language such as “retrieve information from [URL],” Gemini often declined to respond, citing limitations. In contrast, when the same question was rephrased more conversationally—e.g., “tell me about this person”—Gemini was more likely to provide a substantive answer. This behavior indicates that Gemini's underlying alignment or intent-detection mechanisms are sensitive to linguistic cues in user instructions (see Figure~\ref{fig:gemini-tone-sensitivity}).

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/screenshot2.png}
        \caption{Gemini declines to respond when asked to "retrieve" information.}
        \label{fig:subfig1}
    \end{subfigure}
    \hspace{0.04\textwidth}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/screenshot1.png}
        \caption{Gemini provides an answer when asked to "tell me about" the subject.}
        \label{fig:subfig2}
    \end{subfigure}
    \caption{Impact of Query Tone on Gemini’s Willingness to Respond. Direct phrasing leads to refusal, while indirect phrasing elicits an answer—even when no webpage policy is present.}
    \label{fig:gemini-tone-sensitivity}
\end{figure}

\paragraph{Retrieval Limitation on Fictional Content}
Gemini exhibited retrieval limitations when dealing with fictional or fabricated webpage content. It consistently failed to retrieve information from websites featuring entirely fictitious entities not indexed or present elsewhere online, despite explicit URLs provided. We infer that Gemini's retrieval logic heavily relies on its pre-existing indexed knowledge and external verification mechanisms, restricting its ability to process purely fabricated content (Figure \ref{fig:gemini-fictional-limitations}).

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/screenshot4.png}
        \caption{GGemini successfully retrieves and summarizes content for a \textbf{real} individual.}
        \label{fig:subfig4}
    \end{subfigure}
    \hspace{0.04\textwidth}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/screenshot3.png}
        \caption{Gemini fails to retrieve content for a \textbf{fictional} person, despite being given the correct URL.}
        \label{fig:subfig3}
    \end{subfigure}
    \caption{Gemini's Retrieval Behavior on Real vs. Fictional Webpages. The model can extract and respond to queries about real entities but fails to retrieve from non-indexed or fictitious sites, even with explicit URLs.}
    \label{fig:gemini-fictional-limitations}
\end{figure}
